Post-Stall Navigation with Fixed-Wing UAVs using Onboard Vision

Recent research has enabled fixed-wing unmanned aerial vehicles (UAVs) to maneuver in constrained spaces through the use of direct nonlinear model predictive control (NMPC). However, this approach has been limited to a priori known maps and ground truth state measurements. In this paper, we present a direct NMPC approach that leverages NanoMap, a light-weight point-cloud mapping framework to generate collision-free trajectories using onboard stereo vision. We first explore our approach in simulation and demonstrate that our algorithm is sufficient to enable vision-based navigation in urban environments. We then demonstrate our approach in hardware using a 42-inch fixed-wing UAV and show that our motion planning algorithm is capable of navigating around a building using a minimalistic set of goal-points. We also show that storing a point-cloud history is important for navigating these types of constrained environments.

==> results.tex <==
\section{Results}

\subsection{Simulated Perception}

The controller parameters were as follows:
\begin{align}
  \vect{Q}&=[25,25,25,50,50,50,2,2,2,2,2,2] \nonumber \\
  \vect{r}&=[0.1,0.1,0.1,25] \nonumber \\
  \vect{Q_f}&=[100,100,100,100,100,100,1,1,1,1,1,1] \nonumber \\
  \vectg{\delta_f}&=[0.5, 0.5, 0.5, 0.5, 0.5, 0.5, 3, 3, 0.5, 0.5, 0.5, 40] \nonumber
\end{align}

A time horizon of $T_H=1s$ and a replanning frequency of 5Hz were used. We used the obstacle distance constraint with a radius of 2.95 meters.

The fixed-wing was successfully able to navigate around the building to the way points using simulated depth camera data. Figure \ref{Fig:gazebo} shows the flight path taken by the fixed-wing overlayed with the obstacle distance constraint radius.

\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{images/gazebo.png}
    \caption{Physical flight path using simulated depth camera data}
  \label{Fig:gazebo}
\end{figure}

\subsection{Control Experiment}

Out of six hardware trials, four were considered successful. In one of these trials, the fixed-wing crashed into a light pole after making it around the building. This crash was caused by inability of the depth sensor to see the pole until the fixed wing was too close to react.

The paths of the successful trials are shown in Figure \ref{Fig:successful}, and the obstacle distance constraint radii are overlayed in Figure \ref{Fig:successful_radius}. Additionally, the search depths of NanoMap queries are shown in Figures \ref{Fig:library_search} and \ref{Fig:library_turn_search}. Similar to the simulation trials, while the majority of the queries depths were from the most recent pointcloud, the optimizer does query quite far back in the NanoMap history.

\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{images/successful_library.png}
    \caption{Physical flight path}
  \label{Fig:successful}
  \centering
  \includegraphics[width=.9\linewidth]{images/successful_radius.png}
    \caption{Obstacle distance constraint radius}
  \label{Fig:successful_radius}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{images/library_search.png}
    \caption{NanoMap search depth queries across all iterations}
  \label{Fig:library_search}
  \centering
  \includegraphics[width=.9\linewidth]{images/library_turn_search.png}
    \caption{NanoMap search depth queries while turning}
  \label{Fig:library_turn_search}
\end{figure}

Two of the hardware trials failed, crashing into the building shortly after turning corners, as shown in Figure \ref{Fig:failed}.  In both of these failure cases, the RRT paths caused the fixed-wing to turn towards the building very late while rounding the corners.  As a result, the depth camera does not observe the part of the wall after the corner, causing new RRT paths to be generated through the apparent gap. This caused infeasible trajectories, leading to crashes.

\begin{figure}[h]
  \centering
  \includegraphics[width=.9\linewidth]{images/failed.png}
    \caption{Failed flight paths}
  \label{Fig:failed}
\end{figure}

\label{sec:results}

